What's in a Latent? Leveraging Diffusion Latent Space for Domain Generalization

Domain Generalization aims to develop models that can generalize to novel and unseen data distributions. In this work, we study how model architectures and pre-training objectives impact feature richness and propose a method to effectively leverage them for domain generalization. Specifically, given a pre-trained feature space, we first discover latent domain structures, referred to as pseudo-domains, that capture domain-specific variations in an unsupervised manner. Next, we augment existing classifiers with these complementary pseudo-domain representations making them more amenable to diverse unseen test domains. We analyze how different pre-training feature spaces differ in the domain-specific variances they capture. Our empirical studies reveal that features from diffusion models excel at separating domains in the absence of explicit domain labels and capture nuanced domain-specific information. On 5 datasets, we show that our very simple framework improves generalization to unseen domains by a maximum test accuracy improvement of over 4% compared to the standard baseline Empirical Risk Minimization (ERM). Crucially, our method outperforms most algorithms that access domain labels during training.

==> common_headers.tex <==
% \usepackage[usenames, dvipsnames]{xcolor}
% % \usepackage[colorlinks, citecolor=RoyalPurple, linkcolor=Mahogany]{hyperref}
\usepackage{soul}
\usepackage{xfrac}
% % \usepackage[small]{caption}
% \usepackage{subcaption}
% \usepackage{url}
% \usepackage{graphicx}
% \usepackage{natbib}
% \usepackage{bibentry}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algorithmic}
% % \usepackage{subcaption}
% \usepackage{breakcites}
% \usepackage{circledsteps}
\usepackage{bbm}
% \usepackage{natbib}
\usepackage{bm}
% % \usepackage[document]{ragged2e}

\usepackage{booktabs} % For professional-looking tables
\usepackage{adjustbox} % For resizing tables
\usepackage{siunitx} % For aligning numbers and using \pm
\usepackage{float} 


% \urlstyle{same}
% % \DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

% % \usepackage{tabularx} % extra features for tabular environment
% % \usepackage{amsmath, amsfonts}  % improve math presentation
% \usepackage{graphicx} % takes care of graphic including machinery
% % \usepackage{cite} % takes care of citations
% \usepackage{tcolorbox}
\usepackage{amsmath}
\usepackage{amsthm}
% \usepackage{multirow}
% \usepackage{amssymb}  
% % \usepackage{tabularx} % extra features for tabular environment
% \usepackage{amsmath}  % improve math presentation
% \usepackage{amsthm}
\usepackage{mathtools}
% \usepackage{makecell}
% % \usepackage{mathabx}
% % \usepackage{dutchcal}
% % \usepackage{mathtools}  % <----- for '\mathrlap' command (necessary)

\newcommand{\x}{{\bf x}}
\newcommand{\bx}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\by}{{\bf y}}
\newcommand{\ty}{{\tilde{\bf y}}}
\newcommand{\w}{{\bf w}}
\newcommand{\bw}{{\bf w}}
\newcommand{\be}{{\bf e}}
\newcommand{\bn}{{\bf n}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bz}{{\bf z}}
\newcommand{\z}{{\bf z}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bepsilon}{{\bm \varepsilon}}
\newcommand{\bvarepsilon}{{\bm \varepsilon}}
\newcommand{\tx}{\tilde{\bm x}}
\newcommand{\ta}{\tilde{\bm a}}
\newcommand{\bxi}{{\bm \xi}}
\newcommand{\bLambda}{{\bm \Lambda}}
\newcommand{\blambda}{{\bm \lambda}}
\newcommand{\balpha}{{\bm \alpha}}
\newcommand{\bupsilon}{{\bm \upsilon}}
\newcommand{\btau}{{\bm \tau}}
\newcommand{\bkappa}{{\bm \kappa}}
\newcommand{\bUpsilon}{{\bm \Upsilon}}
\newcommand{\bDelta}{{\bm \Delta}}
\newcommand{\btLambda}{{\widetilde{\bm \Lambda}}}
\newcommand{\btmu}{{\widetilde{\bm \mu}}}
\newcommand{\btu}{{\widetilde{\bf u}}}
\newcommand{\bttheta}{{\widetilde{\bm \theta}}}
\newcommand{\bPhi}{{\bm \Phi}}
\newcommand{\bpsi}{{\bm \psi}}
\newcommand{\bPsi}{{\bm \Psi}}
\newcommand{\btPhi}{{\widetilde{\bm \Phi}}}
\newcommand{\bEpsilon}{\bm{\mathcal E}}
\newcommand{\bh}{{\bf h}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bU}{{\bf U}}
\newcommand{\btk}{{\widetilde{\bf k}}}
\newcommand{\bH}{{\bf H}}
\newcommand{\bW}{{\bf W}}
\newcommand{\bG}{{\bf G}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bK}{{\bf K}}
\newcommand{\btK}{{\widetilde{\bf K}}}
\newcommand{\bV}{{\bf V}}
\newcommand{\bQ}{{\bf Q}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bA}{{\bf A}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bZ}{{\bf Z}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bs}{{\bf s}}
\newcommand{\bq}{{\bf q}}
\newcommand{\br}{{\bf r}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bL}{{\bf L}}
\newcommand{\ba}{{\bf a}}
\newcommand{\bone}{\mathbbm{1}}
\newcommand{\bI}{{\bf I}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bN}{{\bf N}}
\newcommand{\btS}{{\widetilde{\bf S}}}
\newcommand{\bSigma}{{\bf \Sigma}}
\newcommand{\bTheta}{{\bf \Theta}}
\newcommand{\bsigma}{{\bm \sigma}}
\newcommand{\bGamma}{{\bf \Gamma}}
\newcommand{\btheta}{{\bm \theta}}
\newcommand{\bomega}{{\bm \omega}}
\newcommand{\bdelta}{{\bm \delta}}
\newcommand{\bpi}{{\bm \pi}}
\newcommand{\bPi}{{\bm \Pi}}
\newcommand{\bmu}{{\bm \mu}}
\newcommand{\bphi}{{\bm \phi}}
\newcommand{\btphi}{\widetilde{\bm \phi}}
\newcommand{\brho}{{\bm \rho}}
\newcommand{\bnu}{{\bm \nu}}
\newcommand{\bbP}{\mathbb P}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbN}{\mathbb N}
\newcommand{\bbS}{\mathbb S}
\newcommand{\bbD}{\mathbb D}
\newcommand{\bbT}{\mathbb T}
\newcommand{\bbE}{\mathbb E}
\newcommand{\bbV}{\mathbb V}
\newcommand{\cX}{\mathcal X}
\newcommand{\cT}{\mathcal T}
\newcommand{\cH}{\mathcal H}
\newcommand{\ctH}{{\widetilde{\mathcal H}}}
\newcommand{\ctO}{{\widetilde{\mathcal O}}}
\newcommand{\cN}{\mathcal N}
\newcommand{\cF}{\mathcal F}
\newcommand{\cW}{\mathcal W}
\newcommand{\cL}{\mathcal L}
\newcommand{\cA}{\mathcal A}
\newcommand{\ctA}{\widetilde{\mathcal A}}
\newcommand{\cR}{\mathcal R}
\newcommand{\cB}{\mathcal B}
\newcommand{\ctZ}{\widetilde{\mathcal Z}}
\newcommand{\cD}{\mathcal D}
\newcommand{\cO}{\mathcal O}
\newcommand{\cM}{\mathcal M}
\newcommand{\cV}{\mathcal V}
\newcommand{\cE}{\mathcal E}
\newcommand{\cZ}{\mathcal Z}
\newcommand{\cC}{\mathcal C}
\newcommand{\cI}{\mathcal I}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cU}{\mathcal U}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cS}{\mathcal S}
\newcommand{\fP}{\mathfrak P}
\newcommand{\fT}{\mathfrak T}
\newcommand{\fK}{\mathfrak K}
\newcommand{\fC}{\mathfrak C}
\newcommand{\fV}{\mathfrak V}
\newcommand{\fR}{\mathfrak R}
\newcommand{\fD}{\mathfrak D}
\newcommand{\fA}{\mathfrak A}
\newcommand{\fs}{\mathfrak s}
\newcommand{\fp}{\mathfrak p}
\newcommand{\cP}{\mathcal P}
\newcommand{\regret}{\mathsf{Regret}}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\kl}{\bbD_{\mathsf{KL}}}
\newcommand{\tv}{\bbD_{\mathsf{TV}}}


% % \DeclareMathOperator{\sign}{sign}
% \newtheorem{theorem}{Theorem}
% \newtheorem{claim}{Claim}
% \newtheorem{corollary}{Corollary}
% \newtheorem{lemma}{Lemma}
% \newtheorem{assumption}{Assumption}
% \newtheorem{proposition}{Proposition}
% \newtheorem{definition}{Definition}
% \newtheorem{fact}{Fact}
% % \theoremstyle{definition}
% \newtheorem{remark}{Remark}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \usepackage{mathtools}
% \DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
% \DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

% \newcommand{\etal}{\textit{et al.}}
\allowdisplaybreaks

==> fig_latex/nmi_timestep.tex <==
\begin{figure}[!h]
    \centering
    {\includegraphics[width=0.9\linewidth]{appendix_imgs/class_domain_nmi_comparison.png}}
    \caption{\footnotesize{\textbf{Effect of noise on class and domain NMI scores for SD-2.1 on PACS and TerraIncognita}. (Left) Class NMI increases for PACS (up to a certain timestep) but decreases for TerraIncognita as noise increases. (Right) Domain NMI decreases for both datasets with increasing noise. Domain NMI is relatively high for PACS at later timesteps. Timestep represents the noise level at a given denoising step, with higher timesteps indicating greater noise. }}\label{fig:nmi_timestep}
\end{figure} 

==> tables_latex/class_nmi_backup.tex <==
% \begin{table}[!t]
% \centering
% \resizebox{0.35\textwidth}{!}{%
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Dataset} & \textbf{DiT} & \textbf{SD-2.1} & \textbf{MAE} & \textbf{CLIP} & \textbf{DINOv2} & \textbf{RN50} \\
% \midrule
% PACS             & 0.08            & 0.08          & 0.11            & 0.05             & 0.15             & 0.29             \\
% VLCS             & 0.12            & 0.15          & 0.17            & 0.01             & 0.11             & 0.39             \\
% TerraInc   & 0.32            & 0.35           & 0.32           & 0.01            & 0.16             & 0.30            \\
% OfficeHome   & 0.16            & 0.22          & 0.28           & 0.10            & 0.23             & 0.59            \\
% DomainNet   & 0.16            & 0.20          & 0.24           & 0.13            & 0.19             & 0.36            \\
% Geode   & X            & X          & X           & X            & X             & X            \\
% \bottomrule
% \end{tabular}}
% \caption{\footnotesize \textbf{Comparison of Class NMI Scores Across Datasets.} In terms of domain separation, a lower class NMI score (along with a high domain NMI score) is desirable, i.e. the latent space does not tend to group classes from different domains together.}
% \label{tab:class_nmi_dataset_comparison}
% \end{table}

\begin{table}[!t]
\centering
\resizebox{0.35\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Dataset} & \textbf{DiT} & \textbf{SD-2.1} & \textbf{MAE} & \textbf{CLIP} & \textbf{DINOv2} & \textbf{RN50} \\
\midrule
PACS             & 0.08            & 0.11          & 0.14            & 0.05             & 0.15             & 0.28             \\
VLCS             & 0.12            & 0.15          & 0.19            & 0.04             & 0.10             & 0.39             \\
TerraInc   & 0.35            & 0.35           & 0.33           & 0.01            & 0.17             & 0.33            \\
OfficeHome   & 0.16            & 0.25          & 0.29           & 0.10            & 0.23             & 0.59            \\
DomainNet   & X            & 0.20          & 0.13           & X            & X             & X            \\
\bottomrule
\end{tabular}}
\caption{\footnotesize \textbf{Comparison of Class NMI Scores Across Datasets.} In terms of domain separation, a lower class NMI score (along with a high domain NMI score) is desirable, i.e. the latent space does not tend to group classes from different domains together.}
\label{tab:class_nmi_dataset_comparison}
\end{table}

==> tables_latex/dino_feat.tex <==
\begin{table}[!t]
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lc}
\toprule
\textbf{Model} & \textbf{Acc} \\
\midrule
\algoname-DiT      & 68.4                  \\
\algoname-SD      & 68.6                  \\
\algoname-DINOv2             & 68.3                     \\
\bottomrule
\end{tabular}}
\caption{\footnotesize \textbf{Domain generalization performance on various pseudo-domain spaces ($\bPsi$) for OfficeHome}.}
\label{tab:oh_gen_spaces}
\end{table}


==> tables_latex/domain_nmi_backup.tex <==
% \begin{table}[!t]
% \centering
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Dataset} & \textbf{DiT} & \textbf{SD-2.1} & \textbf{MAE} & \textbf{CLIP} & \textbf{DINOv2} & \textbf{RN50} \\
% \midrule
% PACS             & \textbf{0.85}            & 0.82           & 0.71            & 0.54             & 0.55             & 0.59             \\
% VLCS             & \textbf{0.58}            & 0.26           & 0.20            & 0.01             & 0.05             & 0.22             \\
% TerraInc   & 0.22            & \textbf{0.35}           & 0.21           & 0.01            & 0.01             & 0.25            \\
% OfficeHome   & 0.25            & 0.22           & 0.10           & 0.12           & \textbf{0.38}             & 0.08           \\
% DomainNet   & \textbf{0.48}            & 0.47           & 0.44           & 0.36           & 0.47             & 0.40           \\
% Geode   & \textbf{0.008}            & 0.004          & 0.003           & 0.001           & 0.003             & 0.002          \\
% Synth-Artists & \textbf{0.89}           &   0.86         & 0.75            & 0.25             & 0.34             & 0.63           \\
% Synth-Photography & 0.35           & \textbf{0.43}           & 0.31            & 0.17             & 0.23             & 0.33           \\
% \bottomrule
% \end{tabular}}
% \caption{\footnotesize \textbf{Comparison of Domain NMI Scores Across Datasets.} The highest domain NMI score varies with the type of domain shifts observed in the data, as noted in Sec~\ref{sec:pretrain_obj}}
% \label{tab:dataset_comparison}
% \end{table}

\begin{table}[!t]
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Dataset} & \textbf{DiT} & \textbf{SD-2.1} & \textbf{MAE} & \textbf{CLIP} & \textbf{DINOv2} & \textbf{RN50} \\
\midrule
PACS             & \textbf{0.85}            & 0.83           & 0.72            & 0.53             & 0.53             & 0.58             \\
VLCS             & \textbf{0.62}            & 0.26           & 0.29            & 0.01             & 0.06             & 0.32             \\
TerraInc         & 0.27            & \textbf{0.38}           & 0.19           & 0.001            & 0.01             & 0.25            \\
OfficeHome       & 0.24            & 0.23           & 0.13           & 0.12           & \textbf{0.38}             & 0.05           \\
DomainNet       & \textbf{X}            & X           & X           & X           & X             & X           \\
Geode           & \textbf{X}            & X          & X           & X           & X             & X          \\
Synth-Artists   & \textbf{X}           & X         & X            & X             & X             & X           \\
Synth-Photography & X           & \textbf{X}           & X            & X             & X             & X           \\
\bottomrule
\end{tabular}}
\caption{\footnotesize \textbf{Comparison of Domain NMI Scores Across Datasets.} The highest domain NMI score varies with the type of domain shifts observed in the data, as noted in Sec~\ref{sec:pretrain_obj}\xavier{updating NMI numbers for kmeans++ and reproducibility}}
\label{tab:dataset_comparison}
\end{table}

==> tables_latex/domain_shifts.tex <==
\begin{table*}[t]
\centering
\scriptsize % Adjusts the font size
\begin{tabular}{lcc}
\hline
\textbf{Dataset}      & \textbf{Type}              & \textbf{Example}       \\ \hline
PACS       & Global and Textural                & monochromatic ``Sketch" images vs rich in color ``Art Painting"      \\
VLCS        & dataset-specific biases           & spatial composition, object size variations (e.g., objects in ``Caltech" are centered in the image)       \\
OfficeHome (OH) & Low-Level Style differences     & bold edges in ``Clipart" vs softer edges in ``Real World" \\
TerraIncognita (TI) & Static Background; Environmental Changes       & foliage specific to each location differs between domains \\ \hline
\end{tabular}
\caption{\textbf{Overview of the Domain Shifts in each dataset}}
\label{tab:domain_shifts}
\end{table*}


==> tables_latex/geode.tex <==
\begin{table}[!t]
\centering
\scriptsize
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Algorithm} & \textbf{EU} & \textbf{AF} & \textbf{SEA} & \textbf{AM} & \textbf{WA} & \textbf{EA} & \textbf{Avg} \\
\midrule
ERM & 92.4  & 89.2 & 90.6 & 91.5 & 91.8 & 89.5 & 90.8 \\
\midrule
\algoname-DiT & 93.3  & 90.0 & 90.6 & 92.3 & 93.1 & 89.5 & \textbf{91.5} \\
\algoname-SD & 92.7  & 89.9 & 90.6 & 91.7 & 92.3 & 89.7 & 91.1 \\
\bottomrule
\end{tabular}}
\vspace{-1.1em}
\caption{\footnotesize \textbf{Performance across different regions on Geode}. The gains in accuracy for {\algoname} provides evidence for its robustness in real-word applications. EU - Europe, AF - Africa, SEA - South East Asia, AM - Americas, WA - West Asia, ES - East Asia. We report the performance on Geode following the default setting of Domainbed (see Sec.~\ref{sec:impl}).\deepti{Unify how the dataset is called everywhere applies to domainbed and geode.}}
\vspace{-1.2em}
\label{tab:regional_performance}
\end{table}


==> tables_latex/models.tex <==
\begin{table}[t]
\centering
\scriptsize % Adjusts the font size
\begin{tabular}{lccc}
\hline
\textbf{Model}           & \textbf{Params} & \textbf{Feature Dim} & \textbf{Architecture}       \\ \hline
ResNet50    & X                        & X                 & CNN \\
CLIP          & X                         & X                 & ViT \\
DINOv2          & X                          & X                  & ViT \\
MAE            & X                         & X                  & ViT \\
Stable Diffusion 2.1 (SD) & X     & X                & CNN  \\
DiT~\cite{}            & X                         & X                 & ViT    \\ \hline
\end{tabular}
\caption{\textbf{Model overview}. Summary of the key attributes for the models evaluated in this study.}
\label{tab:models}
\end{table}


==> tables_latex/sd_versions.tex <==
\begin{table}[!t]
\centering
\resizebox{0.22\textwidth}{!}{%
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{Domain NMI}} \\
\cmidrule(lr){2-3}
 & \textbf{PACS} & \textbf{TerraInc} \\
\midrule
SD-1.5  & 0.78  & X  \\
SD-2.1  & 0.82  &  0.55  \\
SDXL    & X  & X  \\
\bottomrule
\end{tabular}}
\caption{\footnotesize \textbf{Comparison of Domain NMI Scores Across Stable Diffusion Variants.}}
\label{tab:sd_comparison}
\end{table}

==> tables_latex/seperation_score.tex <==
\begin{table}[!h]
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Dataset} & \textbf{DiT} & \textbf{SD} & \textbf{MAE} & \textbf{CLIP} & \textbf{DINOv2} & \textbf{RN50} \\
\midrule
PACS             & \textbf{0.79}            & 0.76          &  0.64           & 0.51             & 0.48             & 0.46             \\
VLCS             & \textbf{0.52}            & 0.23          & 0.17            & 0.01             & 0.05             & 0.16             \\
TerraInc   & 0.17            & \textbf{0.41}           & 0.16           & 0.01            & 0.01             & 0.19            \\
OfficeHome   & 0.22            &  0.18         & 0.08           & 0.11           & \textbf{0.31}             & 0.05            \\
\bottomrule
\end{tabular}}
\caption{\footnotesize \textbf{Comparison of Domain-Class Separation Scores (DCSS) Across Datasets.} \text{DCSS} = \text{Domain NMI} \, / \, (1 + \text{Class NMI}), provides a way to conflate high domain nmi and low class nmi into a single score. The scores follow the trend of the Domain NMI scores, further emphasizing that high domain separation leads to class invariant structures.\xavier{RECOMPUTE THIS!}}
\label{tab:class_nmi_dataset_comparison}
\end{table}
